Evaluating Disentanglement in Generative Models Without Knowledge of Latent Factors

Probabilistic generative models provide a flexible and systematic framework for learning the underlying geometry of data. However, model selection in this setting is challenging, particularly when selecting for ill-defined qualities such as disentanglement or interpretability. In this work, we address this gap by introducing a method for ranking generative models based on the training dynamics exhibited during learning. Inspired by recent theoretical characterizations of disentanglement, our method does not require supervision of the underlying latent factors. We evaluate our approach by demonstrating the need for disentanglement metrics which do not require labels\textemdash the underlying generative factors. We additionally demonstrate that our approach correlates with baseline supervised methods for evaluating disentanglement. Finally, we show that our method can be used as an unsupervised indicator for downstream performance on reinforcement learning and fairness-classification problems.

==> algorithms/disagreement.tex <==
\begin{algorithm}[t]
\caption{\textbf{\algname{}} training procedure}
\begin{flushleft}
\textbf{Input:} Training data $\mathcal{D}$, validation-data set $\mathcal{\hat{D}}$, max iterations $T$, learning rates $\alpha, \beta$\\
\textbf{Output:} Classifier parameters $\theta$
\end{flushleft}
\begin{algorithmic}[1]
\State $t \gets 0$
\State Initialize $\theta_0$, $\mu_0$, $w_{0} = \omega_{\mu_{0}}(\Delta)$
\For{$t\leq T$}    
    \State $(X,y) \sim \mathcal{D}$, $(\hat{X},\hat{y}) \sim \mathcal{\hat{D}}$
    
\State $\tilde{\theta}_t \gets \theta_t - \beta\cdot\nabla_\theta\hat{\mathcal{L}}_\textrm{tr}|_{\tilde{\theta}_t, w_t}$
    \State $\mu_{t+1} = \mu_t - \alpha\nabla_\mu\hat{\mathcal{L}}_{\textrm{val}}|_{\theta_t, w_t}$ 
    \Comment{compute $\nabla_\mu\hat{\mathcal{L}}_{\textrm{val}}|_{\tilde{\theta}_t,w_t}$ via backpropagation according to Eq.~(\ref{eq:wupdate}})
    %\Comment{compute $\nabla_\mu\hat{\mathcal{L}}_{\textrm{val}}|_{\theta_t, w_t}$ according to Alg. \ref{alg:reweighting_proc}}

    \State compute $w_{t+1} = \omega_{\mu_{t+1}}(\Delta)$
    \Comment{compute $\Delta$ with respect to $\theta_t$ according to Def~\ref{def:mcm}}
    \State $\theta_{t+1} = \theta_{t} - \beta\nabla_{\theta}\hat{\mathcal{L}}_{\textrm{tr}}|_{\theta_t, w_{t+1}}$
\EndFor
\State \Return $\theta_T$
\end{algorithmic}
\label{alg:training_proc}
\end{algorithm}

==> tables/architecture.tex <==
\begin{table}[]
\caption{Encoder and Decoder implementation details.}
\label{tab:arch}
\begin{center}
\begin{tabular}{l}
\hline
Encoder           \\
\hline 
Input: $64 \times 64\times \text{number of channels}$ \\
$4\times 4$ conv, $32$ ReLU, stride $2$ \\
$4\times 4$ conv, $32$ ReLU, stride $2$ \\
$4\times 4$ conv, $64$ ReLU, stride $2$ \\
$4\times 4$ conv, $64$ ReLU, stride $2$ \\
FC $256$, F$2$ $2\times 10$ \\
\hline
Decoder \\
\hline
$4\times 4$ deconv, number of channels, stride $2$ \\
Input: $\mathbb{R}^d$ \\
FC, $256$ ReLU \\
FC, $4\times 4\times 64$ ReLU \\
FC, $4\times 4$ conv, $64$ ReLU, stride $2$ \\
FC, $4\times 4$ conv, $32$ ReLU, stride $2$ \\
$4\times 4$ deconv, $32$ ReLU, stride $2$\\ \hline
\end{tabular}
\end{center}
\end{table}

==> tables/architecture2.tex <==
\begin{table*}[t]
\caption{Encoder and Decoder implementation details for all models}
\label{tab:arch}
\begin{center}
\begin{tabular}{ll}
\hline
Encoder          & Decoder          \\
\hline 
Input: $64 \times 64\times \text{number of channels}$ & Input: $\mathbb{R}^d$ \\
$4\times 4$ conv, $32$ ReLU, stride $2$ & FC, $256$ ReLU \\
$4\times 4$ conv, $32$ ReLU, stride $2$ & FC, $4\times 4\times 64$ ReLU \\
$4\times 4$ conv, $64$ ReLU, stride $2$ & FC, $4\times 4$ conv, $64$ ReLU, stride $2$ \\
$4\times 4$ conv, $64$ ReLU, stride $2$ & FC, $4\times 4$ conv, $32$ ReLU, stride $2$ \\
FC $256$, F$2$ $2\times 10$ & $4\times 4$ deconv, $32$ ReLU, stride $2$\\
& $4\times 4$ deconv, number of channels, stride $2$ \\
\end{tabular}
\end{center}
\vspace{-0.8cm}
\end{table*}

==> tables/hyperparameters.tex <==
\begin{table}[h]
\caption{Common hyperparameters}
\label{tab:hyperparam}
\begin{center}
\begin{tabular}{ll}
\hline
Parameter          & Values          \\
\hline 
Batch size & $[32, 64, 128, 256]$ \\
Latent space dimension & $[2, 4, 8, 16, 32]$ \\
Optimizer & SGD \\
Learning rate & $[0.1, 0.01, 0.001]$ \\
Momentum coefficient & $0.9$ \\
Decoder & Bernoulli \\
Weight initialization & Glorot Normal for $W$s, Normal for $b$s  \\
Random seed & $[0,1,2,3,4]$
\end{tabular}
\end{center}
\end{table}
